Temperature Balancing, Layer-wise Weight Analysis, and Neural Network Training

Regularization in modern machine learning is crucial, and it can take various forms in algorithmic design: training set, model family, error function, regularization terms, and optimizations. In particular, the learning rate, which can be interpreted as a temperature-like parameter within the statistical mechanics of learning, plays a crucial role in neural network training. Indeed, many widely adopted training strategies basically just define the decay of the learning rate over time. This process can be interpreted as decreasing a temperature, using either a global learning rate (for the entire model) or a learning rate that varies for each parameter. This paper proposes TempBalance, a straightforward yet effective layer-wise learning rate method. TempBalance is based on Heavy-Tailed Self-Regularization (HT-SR) Theory, an approach which characterizes the implicit self-regularization of different layers in trained models. We demonstrate the efficacy of using HT-SR-motivated metrics to guide the scheduling and balancing of temperature across all network layers during model training, resulting in improved performance during testing. We implement TempBalance on CIFAR10, CIFAR100, SVHN, and TinyImageNet datasets using ResNets, VGGs, and WideResNets with various depths and widths. Our results show that TempBalance significantly outperforms ordinary SGD and carefully-tuned spectral norm regularization. We also show that TempBalance outperforms a number of state-of-the-art optimizers and learning rate schedulers.

==> sections/Algorithm.tex <==
\vspace{-3mm}
\section{The \ourmethod Algorithm}
\label{sec:TempBalacne}
\vspace{-2mm}

\begin{figure}[t] 
    \centering
     \begin{subfigure}{0.99\textwidth}
        \includegraphics[width=\textwidth]{figs/overview/TB_system_design_v3.pdf}
    \end{subfigure}
     \caption{The pipeline diagram of \ourmethod. In each epoch, \ourmethod undergoes two steps: (a) Performing ESD analysis on all layers and employing PL fitting to derive the layer-wise \ALPHAHILL, and (b) Using the layer-wise \ALPHAHILL to assign learning rates to each layer using an assignment function.}
     \label{fig:Tempbalance}
\end{figure}

In this section, we introduce our simple yet effective method \ourmethod, based on the \ALPHAHILL metric from HT-SR Theory. 
For a NN, different layers tend to have different values for \ALPHAHILL, \citep{martin2017rethinking, martin2018implicit_JMLRversion}: 
a layer with a larger \ALPHAHILL indicates that layer is relatively undertrained, while 
a layer with a smaller \ALPHAHILL indicates that layer is relatively overtrained.
A natural idea is to adjust the degree of learning among different layers to get a balance: for a layer whose \ALPHAHILL is too large, we could assign a larger learning rate to accelerate its learning, and vice versa.
The intuition of our method is transferring one layer’s learning rate to another and hence, \ourmethod. The pipeline is in Figure~\ref{fig:Tempbalance}.



\begin{algorithm}[t] 
	\caption{\ourmethod}
	\label{alg:algorithm1}
	\KwIn{$M$: Deep NN, \quad $T$: Total training epoch, \quad ${t}$: Current epoch,  \quad  
    $\alpha^{i}_t$: $i_\text{th}$ layer's \ALPHAHILL at epoch $t$, \quad $\eta_t$: Baseline global learning rate at epoch $t$, \quad \quad \quad \quad
   $s_{1}, s_{2}$: Minimum and maximum scaling ratio,  \quad $f_t$: Learning rate schedule function
 }
	\BlankLine

	
         Initialize model $M$;
         
		\For{$t \gets 0$ to $T$}{
                
			Compute $\alpha^{i}_t$ for all layers using the Hill estimator;
   
			Leverage all $\alpha^{i}_t$ and adopt $f_t$ in~\eqref{eqn:learning_rate_mapping} to assign per-layer learning rate $f_t(i)$ between $s_1 \eta_t$ and $s_2 \eta_t$ for the next epoch;

              Update the optimizer for the next epoch;
   
		}
		 
\end{algorithm}

We provide the details of \ourmethod in Algorithm ~\ref{alg:algorithm1}.
Based on \ALPHAHILL in different layers, we use the learning rate schedule function $f_t$ to map the $i$-{th} layer to a particular learning rate $f_t(i)$ in epoch $t$. We adopt $f_t$ as a linear map between the layer-wise \ALPHAHILL and the final layer-wise learning rate, which has the following formula:

\begin{equation}\label{eqn:learning_rate_mapping}
f_{t}(i)=\eta_t\cdot \left[\frac{\alpha^{i}_t-\alpha^\text{min}_t}{\alpha^\text{max}_t-\alpha^\text{min}_t}(s_2-s_1) +s_1\right],
\end{equation}
where $\eta_{t}$ means the base global learning rate in epoch $t$, $(s_1, s_2)$ are the minimum and maximum learning rate scaling ratio relative to $\eta_{t}$, $\alpha^{i}_{t}$ represents the layer $i$'s \ALPHAHILL at the beginning of epoch $t$, and $(\alpha^\text{min}_{t},\alpha^\text{max}_t)$ denote the minimum and maximum \ALPHAHILL across all the layers in epoch $t$.
Using \eqref{eqn:learning_rate_mapping}, we ensure that the new learning rate $f_{t}(i)$ is a scaled version of the original base learning rate $\eta_{t}$ and is always inside the interval $[s_1\eta_{t}, s_2\eta_{t}]$.
Note that $(s_1, s_2)$ serves as tunable hyperparameters in our method. 
We conducted ablation studies on it, which are detailed in Appendix~\ref{sec:app-ablation-study}.
The hyperparameter values used across all experiments can be found in Appendix~\ref{app:hyper_parameter}.
Our studies reveal that the optimal results are usually achieved around (0.5, 1.5).



To fit the PL distribution $p(\lambda)$ defined in~\eqref{eqn:ALPHA}, we use the Hill estimator~\citep{hill1975simple, xiao2023heavy}.
(It is not the best estimator for fine-scale diagnostics based on HT-SR Theory~\citep{martin2018implicit_JMLRversion,martin2020predicting_NatComm}, but it is robust, and it suffices for our purposes.)
For the $i$-th layer, suppose the weight matrix is $\mathbf{W}_i$ and the correlation matrix $\mathbf{W}_i^\top\mathbf{W}_i$ has ascending eigenvalues $\lbrace \lambda_{i} \rbrace_{i=1}^n$. Then, the Hill estimator calculates \ALPHAHILL using the following: 
\begin{equation}\label{eqn:hill_estimator}
\ALPHAHILL= 1+\frac{k}{(\sum_{i=1}^k ln\frac{\lambda_{n-i+1}}{\lambda_{n-k}})},
\end{equation}
where $k$ is the adjustable parameter.
We adopt $k=\frac{n}{2}$ in  our experiments.
Note that changing $k$ essentially changes the lower eigenvalue threshold $\lambda_\text{min}$ for (truncated) PL estimation, as shown by the vertical black line in Figure~\ref{fig:PL_examples}.
Choosing $k=\frac{n}{2}$ means using the largest half of the eigenvalues to estimate the slope.
We empirically find that fixing $k$ for all layers leads to more stable performance than searching $k$ for different layers (e.g., optimizing $k$ using the Kolmogorov–Smirnov test~\citep{alstott2014powerlaw}, as is needed for other applications of HT-SR Theory~\citep{martin2018implicit_JMLRversion,martin2020predicting_NatComm}).

One advantage of mapping \ALPHAHILL to learning rates using~\eqref{eqn:learning_rate_mapping} is that the scale of \ALPHAHILL is unimportant, i.e., linearly scaling \ALPHAHILL arbitrarily does not change the learning rate assignment because the linear scaling cancels each other in~\eqref{eqn:learning_rate_mapping}.
This can maximally reduce the artifact of estimating the ESD PL exponent/slope due to estimation noise, which has been found to be a tricky issue in practice~\citep{MM21a_simpsons_TR,martin2018implicit_JMLRversion}.





==> sections/Experiments.tex <==
\vspace{-3mm}
\section{Empirical results}
\label{sec:experiments}
\vspace{-2mm}

In this section, 
we 
give full details of the experimental setup (Section~\ref{sec:set_up}) 
and 
compare our method \ourmethod to a few baselines (Section~\ref{sec:main_result}), 
and then 
(Section~\ref{sec:ablation_studies}) 
we perform ablation studies on varied initial learning rates, model widths, HT-SR layer-wise metrics, and PL fitting~methods.\looseness-1

\input{sections/Experiments_setup.tex}
\input{sections/Experiments_baseline}
\input{sections/Experiments_ablation}


==> sections/Experiments_ablation.tex <==

\vspace{-2mm}
\subsection{Corroborating results and ablation studies.}
\label{sec:ablation_studies}
\vspace{-1mm}

In addition to the main results (Figures~\ref{fig:main_result} and~\ref{fig:compare_results}), we provide corroborating results and ablation~studies.


\textbf{Experiment one: tuning initial learning rate $\eta_0$}. 
We train models from scratch using \ourmethod versus \texttt{CAL} with various initial learning rates, comparing \ourmethod and the \texttt{CAL} baseline when both methods are allowed to search for the optimal hyperparameters.
We again use ResNet18, ResNet34, VGG16 and VGG19 as our architectures and show results on CIFAR100.
Results in Figure~\ref{fig:tune_learning_rate} show that \ourmethod achieves a higher test accuracy than \texttt{CAL} for both ResNet and~VGG. 



\textbf{Experiment two: varying channel width.}
We view the fraction of model width in Experiment one as ``$100\%$,'' and we experiment with models with varied widths in $[50\%,100\%,150\%]$. 
We again used ResNet18, ResNet34, VGG16 and VGG19, and trained on CIFAR100, and we grid search for the optimal learning rate for each width to get the best accuracy.
Results in Figure~\ref{fig:tune_model_width} show we find that \ourmethod outperforms the baseline for all widths.

\begin{figure}
\centering
\begin{subfigure}{0.3\linewidth} 
\includegraphics[width=\linewidth,keepaspectratio]{figs/ablation/abl_lr_legend.png} 
\end{subfigure} \\
\begin{subfigure}{0.24\linewidth}
\includegraphics[width=\linewidth,keepaspectratio]{figs/ablation/cifar_resnet18_lr.png} 
\caption{ResNet18, CIFAR100}
\end{subfigure}
\begin{subfigure}{0.24\linewidth}
\includegraphics[width=\linewidth,keepaspectratio]{figs/ablation/cifar_resnet34_lr.png}
\caption{ResNet34, CIFAR100}
\end{subfigure}
\begin{subfigure}{0.24\linewidth}
\includegraphics[width=\linewidth,keepaspectratio]{figs/ablation/cifar_vgg16_lr.png} 
\caption{VGG16, CIFAR100}
\end{subfigure}
\begin{subfigure}{0.24\linewidth}
\includegraphics[width=\linewidth,keepaspectratio]{figs/ablation/cifar_vgg19_lr.png} 
\caption{VGG19, CIFAR100}
\end{subfigure}
\caption{{\bf (Tuning initial learning rate).} 
Comparing the test accuracy of \ourmethod (red) and \texttt{CAL} baseline (blue) for varying initial learning rate.
Our method \ourmethod outperforms \texttt{CAL} for both ResNet and VGG trained on CIFAR100.
All results are obtained by running five random seeds.
\label{fig:tune_learning_rate}  
}
\end{figure}

\begin{figure}
\centering
\begin{subfigure}{0.3\linewidth} 
\includegraphics[width=\linewidth,keepaspectratio]{figs/ablation/abl_lr_legend.png} 
\end{subfigure} \\
\begin{subfigure}{0.24\linewidth}
\includegraphics[width=\linewidth,keepaspectratio]{figs/ablation/cifar_resnet18_width_new.png} 
\caption{ResNet18, CIFAR100}
\end{subfigure}
\begin{subfigure}{0.24\linewidth}
\includegraphics[width=\linewidth,keepaspectratio]{figs/ablation/cifar_resnet34_width_new.png}
\caption{ResNet34, CIFAR100}
\end{subfigure}
\begin{subfigure}{0.24\linewidth}
\includegraphics[width=\linewidth,keepaspectratio]{figs/ablation/cifar_vgg16_width_new.png} 
\caption{VGG16, CIFAR100}
\end{subfigure}
\begin{subfigure}{0.24\linewidth}
\includegraphics[width=\linewidth,keepaspectratio]{figs/ablation/cifar_vgg19_width_new.png} 
\caption{VGG19, CIFAR100}
\end{subfigure}

\caption{{\bf (Different widths).} Comparing \ourmethod and the \texttt{CAL} baseline for different network widths. 
Our method \ourmethod consistently outperforms the \texttt{CAL} baseline across various network widths for both ResNet and VGG trained on CIFAR100. 
All results are obtained by running five random seeds.
}
\label{fig:tune_model_width}
\end{figure}


\begin{figure}[!th]
\centering
\begin{subfigure}{0.75\linewidth} 
\includegraphics[width=\linewidth,keepaspectratio]{figs/ablation/metrics/abl_metric_legend.png} 
\end{subfigure} \\
\begin{subfigure}{0.24\linewidth}
\includegraphics[width=\linewidth,keepaspectratio]{figs/ablation/metrics/cifar_resnet18_metrics.png} 
\caption{ResNet18, CIFAR100}
\end{subfigure}
\begin{subfigure}{0.24\linewidth}
\includegraphics[width=\linewidth,keepaspectratio]{figs/ablation/metrics/cifar_resnet34_metrics.png}
\caption{ResNet34, CIFAR100}
\end{subfigure}
\begin{subfigure}{0.24\linewidth}
\includegraphics[width=\linewidth,keepaspectratio]{figs/ablation/metrics/cifar_vgg_cifar16_metrics.png} 
\caption{VGG16, CIFAR100}
\end{subfigure}
\begin{subfigure}{0.24\linewidth}
\includegraphics[width=\linewidth,keepaspectratio]{figs/ablation/metrics/cifar_vgg_cifar19_metrics.png} 
\caption{VGG19, CIFAR100}
\end{subfigure}

\caption{{\bf (Different HT-SR metrics).}
Comparing \ALPHAHILL with multiple HT-SR metrics. 
\ALPHAHILL achieves the best test accuracy among these metrics. 
All results are obtained by running five random seeds. 
\vspace{-4mm}}
\label{fig:ablation_metrics}
\end{figure}

\begin{figure}[!th]
\centering
\begin{subfigure}{0.24\linewidth}
\includegraphics[width=\linewidth,keepaspectratio]{figs/ablation/fitting_types/resnet_18_1_cifar100_0.1.png} 
\caption{ResNet18, CIFAR100}
\end{subfigure}
\begin{subfigure}{0.24\linewidth}
\includegraphics[width=\linewidth,keepaspectratio]{figs/ablation/fitting_types/resnet_34_1_cifar100_0.1.png} 
\caption{ResNet34, CIFAR100}
\end{subfigure}
\begin{subfigure}{0.24\linewidth}
\includegraphics[width=\linewidth,keepaspectratio]{figs/ablation/fitting_types/vgg_cifar_16_1_cifar100_0.1.png} 
\caption{VGG16, CIFAR100}
\end{subfigure}
\begin{subfigure}{0.24\linewidth}
\includegraphics[width=\linewidth,keepaspectratio]{figs/ablation/fitting_types/vgg_cifar_19_1_cifar100_0.1.png} 
\caption{VGG19, CIFAR100}
\end{subfigure}
\caption{\textbf{(Varying PL fitting method to determine the $\lambda_\text{min}$).} Results of using different PL fitting methods. The blue bar plot and the left $y$-axis label denote the test accuracy (higher the better), and the red line plots and the right $y$-axis label denote the time in seconds of using \ourmethod once (lower the better).
Our design (\texttt{Median}) used in the proposed method achieves higher test accuracy and takes lower computation times compared to $\texttt{Goodness-of-fit}$ and $\texttt{Fix-finger}$. The test accuracy is averaged over five random seeds and computation time is averaged over ten times.  
}
\label{fig:alpha-fit-ablation}
\end{figure}


\textbf{Experiment three: varying HT-SR metric}. 
We use different HT-SR metrics to assign layer-wise learning rates. That is, we replace the layer-wise \ALPHAHILL in~\eqref{eqn:learning_rate_mapping} with other HT-SR metrics including \texttt{SpectralNorm} and \texttt{AlphaWeighted}~\citep{martin2020predicting_NatComm}. Results in Figure~\ref{fig:ablation_metrics} show that \ALPHAHILL achieves the optimal test accuracy.

\textbf{Experiment four: varying PL fitting methods.}
The HT-SR metric \ALPHAHILL is derived through PL fitting, which is influenced by the choice of hyperparameter $\lambda_\text{min}$. 
More specifically, this involves determining the adjustable parameter $k$ as per Equation~\ref{eqn:hill_estimator}. 
Past research has employed various methods to select $\lambda_\text{min}$ based on the task, such as performance prediction. For instance, \citet{clauset2009power, martin2020predicting_NatComm} choose $\lambda_\text{min}$ that aligns with the best fit according to the Kolmogorov-Smirnov  statistic~\cite{alstott2014powerlaw}, a method termed $\texttt{Goodness-of-fit}$. Meanwhile, \citet{yang2022evaluating} adopted the $\texttt{Fix-finger}$ approach, which identifies $\lambda_\text{min}$ at the peak of the ESD.
In our study, we designate $\lambda_\text{min}$ as the median of all eigenvalues present in the ESD for \ourmethod. 
As depicted in Figure~\ref{fig:alpha-fit-ablation}, our fitting method, termed $\texttt{Median}$, not only ensures optimal test accuracy but also notably decreases computation time. 
This shows that this PL fitting method is suited for the design of learning rate schedulers that demand low computation overhead.

\textbf{Empirical analysis results.} 
We conduct an empirical analysis of \ourmethod to discuss why it provides improvement.
Our first analysis involves visualization to demonstrate how \ourmethod effectively regularizes ESDs by scheduling the learning rate (see Appendix~\ref{app:visualization}). 
The second analysis strengthens the connections between \ourmethod and HT structure, illustrating that the observed improvements are not due to indirectly addressing other training issues, such as gradient excursions~\cite{pascanu2013difficulty} (see Appendix~\ref{app:grad-ex}). 

\textbf{Corroborating results on other tasks.} We extend our evaluation of \ourmethod to two additional tasks: object detection and language modeling, the details of which can be found in Appendix~\ref{app:more-tasks}. Across these tasks, \ourmethod consistently outperforms the baseline \texttt{CAL} in terms of generalization.\looseness-1
















==> sections/Experiments_baseline.tex <==
\begin{figure}
    \centering
    \begin{subfigure}{0.7\linewidth} 
    \includegraphics[width=\linewidth,keepaspectratio]{figs/main_results/method_legend.png} 
    \end{subfigure} \\
    \centering
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{figs/main_results/cifar100/cifar100_resnet18_best.png}
    \caption{ResNet18, CIFAR100}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{figs/main_results/cifar100/cifar100_resnet34_best.png}
        \caption{ResNet34, CIFAR100}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{figs/main_results/cifar100/cifar100_VGG16_best.png}
        \caption{VGG16, CIFAR100}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{figs/main_results/cifar100/cifar100_VGG19_best.png}
        \caption{VGG19, CIFAR100}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{figs/main_results/tinyimagenet/tiny_resnet18_best.png}
    \caption{ResNet18, TIN}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{figs/main_results/tinyimagenet/tiny_resnet34_best.png}
        \caption{ResNet34, TIN}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{figs/main_results/tinyimagenet/tiny_wrn16_8_best.png}
        \caption{WRN16-8, TIN}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{figs/main_results/tinyimagenet/tiny_wrn28_6_best.png}
        \caption{WRN28-6, TIN}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{figs/main_results/cifar10/cifar10_resnet18_best.png}
    \caption{ResNet18, CIFAR10}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{figs/main_results/cifar10/cifar10_vgg16_best.png}
        \caption{VGG16, CIFAR10}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{figs/main_results/svhn/svhn_resnet18_best.png}
        \caption{ResNet18, SVHN}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{figs/main_results/svhn/svhn_vgg16_best.png}
        \caption{VGG16, SVHN}
    \end{subfigure}
    \caption{{\bf (Main result).} Comparing our method \ourmethod (\texttt{TB}) to \texttt{CAL} and \texttt{SNR}.
    Our method \ourmethod outperforms \texttt{CAL} and \texttt{SNR} in almost all the settings except for VGG19 and ResNet 34 on CIFAR 100.
    For all experiments, combining \ourmethod and \texttt{SNR} (\texttt{TB}+\texttt{SNR}) yields the best performance. All baselines are carefully tuned. All results are obtained by running five random seeds.
    See Appendix~\ref{app:hyper_parameter} for the details in all hyperparameters.}
    \label{fig:main_result}
\end{figure}


\begin{figure}[!h]
    \begin{subfigure}{0.48\textwidth}
    \includegraphics[width=\textwidth]{figs/compare/cifar_resnet18_comparebaseline.png}
    \caption{ResNet18, CIFAR100}
    \end{subfigure}
    \begin{subfigure}{0.48\textwidth}
    \includegraphics[width=\textwidth]{figs/compare/cifar_resnet34_comparebaseline.png}
    \caption{ResNet34, CIFAR100}
    \end{subfigure}
    
    \caption{{\bf (More baseline optimizers).} Comparing our method \ourmethod (\texttt{TB}) to cosine annealing (\texttt{CAL}) baseline and other state-of-the-art optimizers and learning rate schedulers for ResNet18 and ResNet34 trained on CIFAR100. Crosses for the same method represent different hyperparameter settings. Each cross represents the mean test accuracy of five random seeds.
    The best performing model thus far is \texttt{TB} combined with \texttt{SGDP}.}
    \label{fig:compare_results}
\end{figure}

\vspace{-2mm}
\subsection{Comparing \ourmethod and multiple baseline methods.}
\label{sec:main_result}
\vspace{-1mm}



First, we compare \ourmethod to two baseline training methods. See results in Figure~\ref{fig:main_result}. 
In the figure, \texttt{CAL} means \texttt{SGD} training with a \texttt{CAL} learning rate schedule, and \texttt{SNR} means \texttt{SGD} trained with spectral norm regularization. 
\texttt{TB} means our method \ourmethod, and \texttt{TB + SNR} means \ourmethod combined with \texttt{SNR}.
All error bars are obtained from five random seeds.
From Figure~\ref{fig:main_result}, we see that \ourmethod outperforms the \texttt{CAL} baseline in all settings. In almost all cases, it performs better than \texttt{SNR} baseline. When \ourmethod does not outperform \texttt{SNR}, combining \texttt{SNR} with \ourmethod leads to better test accuracy.

Second, we compare our method to a number of optimizers and learning rate schedulers that are not necessarily related to ESD of weights.
These include \texttt{SGDR}~\citep{loshchilovsgdr}, \texttt{SGDP}~\citep{heo2021adamp}, \texttt{Lookahead}~\citep{zhang2019lookahead} and \texttt{LARS}~\citep{you2017scaling,you2018imagenet}, and we compare these baselines with \ourmethod for ResNet18 and ResNet34 trained on CIFAR100.
\texttt{SGDR} is stochastic gradient descent with warm restarts.
\texttt{SGDP} modifies the ordinary \texttt{SGD} to compensate for the effect of increasing weight norm.
\texttt{Lookahead}~\cite{zhang2019lookahead} modifies \texttt{SGD} by letting each gradient update approximate the future trajectory of multiple updates.
\texttt{LARS} assigns layer-wise learning rates based on the so-called ``trust-ratio'' and is the closest to our method.
Results in Figure~\ref{fig:compare_results} show that \ourmethod outperforms these baselines, and \ourmethod combined with \texttt{SGDP} is the best-performing method. The crosses on each column represent training runs with different hyperparameters. Note that there are several other methods based on modifying the \texttt{Adam} optimizer~\citep{kingma2014adam}, such as \texttt{AdamW}~\citep{loshchilovdecoupled}, \texttt{AdamP}~\citep{heo2021adamp} and \texttt{LAMB}~\citep{You2020Large}.
However, we do not find them to provide better results than the \texttt{SGD} baseline with cosine annealing (\texttt{CAL} in Figure~\ref{fig:compare_results}). The results are detailed in Appendix~\ref{app:more-baseline}.







